G-CNN: an Iterative Grid Based Object Detector

We introduce G-CNN, an object detection technique based on CNNs which works without proposal algorithms. G-CNN starts with a multi-scale grid of fixed bounding boxes. We train a regressor to move and scale elements of the grid towards objects iteratively. G-CNN models the problem of object detection as finding a path from a fixed grid to boxes tightly surrounding the objects. G-CNN with around 180 boxes in a multi-scale grid performs comparably to Fast R-CNN which uses around 2K bounding boxes generated with a proposal technique. This strategy makes detection faster by removing the object proposal stage as well as reducing the number of boxes to be processed.

==> defs.tex <==
\usepackage{amsfonts}
\usepackage{amsmath}

% Add the period after section numbers.  Adjust spacing.
\newcommand{\Section}[1]{\vspace{-8pt}\section{\hskip -1em.~~#1}\vspace{-3pt}}
\newcommand{\SubSection}[1]{\vspace{-3pt}\subsection{\hskip -1em.~~#1}
        \vspace{-3pt}}

\newcommand{\psfiguret}[2]
{
  \begin{tabular}{c}
    \psfig{figure=#1,width=#2in}
  \end{tabular}
}

\newcommand{\norm}
\newcommand{\p}{p}
\newcommand{\x}{\vec{x}}
\newcommand{\y}{\vec{y}}
\newcommand{\q}{q}
\newcommand{\W}{W}
\newcommand{\w}{\vec{w}}
\newcommand{\f}{f}
\newcommand{\loss}{\ell}
\newcommand{\fw}{f_{w}}
\newcommand{\bnd}{b}

\newcommand{\Pset}{{\cal P}}
\newcommand{\Qset}{{\cal Q}}

\newcommand{\point}{p}
\newcommand{\qpoint}{q}


\newsavebox{\savepar}
\newenvironment{boxit}{\begin{lrbox}{\savepar}
  \begin{minipage}[b]{1in}}
  {\end{minipage}\end{lrbox}\fbox{\usebox{\savepar}}}


\newcommand{\Heading}[1]{\hspace{-\parindent}{\bf #1}\\}
\newcommand{\1}[1]{\mathds{1}_{[#1]}}
\newcommand{\trans}[1]{{#1}^{\ensuremath{\mathsf{T}}}}
\newcommand{\transs}[1]{{#1}^{\ensuremath{\!\mathsf{T}}}}


\def\vec#1{{\bf #1}}
\def\mat#1{{#1}}

\def\Real{\mathbb{R}}
\def\grad{{\mathbf \nabla}}


\newcommand{\pairloss}{\ell_{\text{pair}}}
\newcommand{\tripleloss}{\ell_{\text{triplet}}}

\newcommand{\Eqref}[1]{Eq.~\ref{#1}} % The '~' stops breaking and gives correct spacing
\newcommand{\tabref}[1]{Table~\ref{#1}}
\newcommand{\secref}[1]{Sec.~\ref{#1}}
\newcommand{\figref}[1]{Fig.~\ref{#1}}

\newcommand{\sign}[0]{\operatorname{sign}\xspace}
\newcommand{\argmax}[1]{\underset{#1}{\operatorname{argmax}}}
%\newcommand{\argmin}[1]{\underset{#1}{\operatorname{argmin}}}
\newcommand{\mean}[1]{\underset{#1}{\operatorname{mean}}}
%\newcommand{\diag}[0]{\operatorname{Diag}}

%% \newcommand{\argmax}{\operatornamewithlimits{argmax}}
%% \underset{x}{\operatorname{argmax}}

%% \newcommand{\argmin}{\operatornamewithlimits{argmin}}
%% \underset{x}{\operatorname{\argmin}}

\def\ie{{\em i.e.,}}
\def\iee{{\em i.e.,}}
\def\eg{{\em e.g.,}}
\def\cf{{\em c.f.,}}
\def\vs{{\em vs.}}

\newcommand{\mohammad}[1]{\textcolor{red}{\textbf{[Mohammad: #1]}}}
\newcommand{\pushmeet}[1]{\textcolor{blue}{\textbf{[Pushmeet: #1]}}}
\newcommand{\david}[1]{\textcolor{blue}{\textbf{[David: #1]}}}
\newcommand{\russ}[1]{\textcolor{green}{\textbf{[Russ: #1]}}}

%\newcommand{\comment}[1]{}
\newcommand{\yrcite}[1]{\cite{#1}}

